On the Carleman ultradifferentiable vectors of a scalar type spectral operator

A description of the Carleman classes of vectors, in particular the Gevrey classes, of a scalar type spectral operator in a reflexive complex Banach space is shown to remain true without the reflexivity requirement. A similar nature description of the entire vectors of exponential type, known for a normal operator in a complex Hilbert space, is generalized to the case of a scalar type spectral operator in a complex Banach space.

==> jinfo.tex <==
\jvolume{21}
\jyear{2015}
\jnumber{4}

